Analytic, Reidemeister and homological torsion for congruence three--manifolds

Starting from the results in math.DG:1212.3161 we prove that for a given Bianchi group, certain natural coefficent modules and a lot of sequences of congruence subgroups of the size of the torsion subgroup of the first homology grows exponentially with the index (we give an explicit rate). We also prove limit multiplicity results for the irreducible components of the space of cuspidal forms.

==> denominators.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Integrality of Eisenstein classes}

We give bounds for the denominators of Eisenstein classes, which will be needed to control the volumes in degree 1. We use $\ovl\QQ,\ovl\ZZ$ to denote the algebraic closure of $\QQ$ and its ring of integers. 

\begin{prop}
There are constants $C,c$ depending on $F$ and $V$ such that for any congruence subgroup $\Gamma'\subset\Gamma=\SL_2(\so_F)$ (we denote by $M$ the hyperbolic manifold $\Gamma'\bs \SL_2(\CC)/K_\infty$) of level $\fri$ there is an integer $N\in\ovl\ZZ$ whose absolute norm $N_0\in\ZZ$ is bounded by $1\le N_0\le C|\fri|^c$ and such that for any $\omega\in H^1(\pl\ovl M;V_{\ovl \ZZ})$ we have 
$$
NE^1(\omega)\in H^1(M;V_{\ovl\ZZ}).
$$
\label{inteis}
\end{prop}

The main idea for the proof, as in \cite[Chapter 6.7]{CV}, is to generate the integral homology using boundary cycles and lifts of so-called modular symbols against which it is feasible to estimate the integrality of Eisenstein classes. Related computations are also given in \cite{Berger}. 


\subsubsection{Notation for the Borel-Serre compactification}
The boundary components of the universal cover of the Borel-Serre compactification of $M$ are indexed by $\PP^1(F)$; we will denote the points on such a boundary component by $(\xi,p)$ where $\xi\in\PP^1(F)$.


\subsubsection{Denominators of differential forms} 
We will denote by $K_f'$ the closure of $\Gamma'$ in $K_f$. Let $f$ be a closed differential form in $\Omega^1(M;V_\CC)$ which represents a class in $H^1(M;V_{\ovl\QQ})$; then its denominator is the smallest $a\in\ovl\ZZ$ such that $a\langle [f], c\rangle_M\in \ovl\ZZ$ for all $c\in H_1(M;V_{\ovl \ZZ}')$ where $V_{\ovl \ZZ}'$ is the dual lattice of $V_{\ovl\ZZ}$ for the determinant pairing $\langle \cdot,\cdot\rangle_V$ on $V_{\ovl\QQ}$. In equivalent terms, the denominator of a class $[f]\in H^1(M;V)$ is equal to the lcm of the denominators of the integrals $\sum_i \int_{c_i}\langle f,v_i\rangle_V$ where $\sum_i c_i\otimes v_i$ runs over the $1$-cycles in $C_*(M;V_\ZZ')$. 


\subsubsection{Decomposition of 1-cycles}
We want to see that we can limit ourselves to computing integrals on boundary cycles together with the following cycles: for $\gamma\in\Gamma'$ and $\xi\in\PP^1(F)\subset\pl\HH^3$ let $c_{\xi,\gamma}$ be the image in $M$ of the geodesic line between the points $\xi$ and $\gamma\xi$. Then $c_{\xi,\gamma}$ is a relative 1-cycle in $\ovl M,\pl\ovl M$ which can be lifted to a 1-cycle ${}^lc_{\xi,\gamma}$ in $\ovl M$ by adding a segment between its two endpoints on the boundary\footnote{The lift is defined only up to a primitive boundary cycle; it will be clear from the arguments below that we need not care about this for our purpose here.}. 

\begin{lemma}
Fix $\xi\in\PP^1(F)$, $x_0\in M$ and let $c_1,\ldots,c_r$ be closed loops based at $x_0$, $v_1,\ldots,v_r\in V_\ZZ$. Suppose that $\sum_i c_i\otimes v_i$ is a cycle, then it is homologous to $b + \sum_i {}^lc_{\xi,\gamma_i}\otimes v_i$ where $b$ is a 1-chain (with coefficients in $V_{\ovl\ZZ}$) supported on cycles in $\pl\ovl M$. 
\label{mod_gen}
\end{lemma}

\begin{proof}
We construct an explicit sum of 2-cells which realises the homology between the two. Fix a geodesic arc $a$ between $x_0$ and the boundary component of $\ovl M$ corresponding to $\xi$; then the endpoint of the lift $\wdt a$ of $a$ starting from $\xi$ finishes (in $\HH^3$) at a lift $\wdt x_0$ of $x_0$ to $\HH^3$. We will denote by $p,q$ the respective endpoints of $\wdt a$ and of $[\xi,\gamma\xi]$ in the boundary component indexed by $\xi$, and by $q'$ the endpoint of the latter on the boundary component corresponding to $\gamma\xi$. Let $\wdt\Delta_i$ be any smoothly embedded disc in $\HH^3$ whose boundary is the loop defined by (when we say 'go from $x$ to $y$' we mean along the geodesic segment $[x,y]$):
\begin{itemize}
\item[(i)] go from $x_0$ to $(\xi,p)$ along $\wdt a$;
 \item[(ii)] go from $(\xi,p)$ to $(\xi,q)$;
\item[(iii)] go from $(\xi,q)$ to $(\gamma_i\xi,q')$;
\item[(iv)] go from $(\gamma_i\xi,q')$ to $(\gamma_i\xi,\gamma_i p)$;
\item[(v)] go from $(\gamma_i\xi,\gamma_i p)$ to $\gamma_i\wdt x_0$ along $\gamma_i\wdt a$;
\item[(vi)] go back to $\wdt x_0$ from $\gamma\wdt x_0$;
\end{itemize}
%This is illustrated in the following figure: ({\bf TBD})
Let $\Delta_i$ be the 2-cell in $M$ image of $\wdt\Delta_i$. The only identifications in $\wdt\Delta_i$ by $\Gamma'$ are between the edges (i) and (v), and thus it follows that:
\begin{equation}
\pl(\Delta_i\otimes v_i) = {}^lc_{\xi,\gamma_i} \otimes v_i + b_i\otimes v_i + a\otimes(v_i-\gamma\cdot v_i) - c_i\otimes v_i
\label{bd_delta}
\end{equation}
where $b_i$ is a boundary 1-cell which comes from the 'excedent' in the edges (ii) and (iv). On the other hand the condition that $\sum_i c_i\otimes v_i$ be a cycle is equivalent to
$$
\sum_i(\gamma\cdot v_i - v_i) = 0
$$
since $\pl(c_i\otimes v_i)=x_0\otimes(\gamma\cdot v_i - v_i)$. Thus it follows from \eqref{bd_delta} that 
$$
\sum_i c_i\otimes v_i = b + \sum_i {}^lc_{\xi,\gamma_i}\otimes v_i + \pl\Delta
$$
where $b$ is the boundary 1-cell $\sum_i b_i\otimes v_i$ and $\Delta=\sum_i\Delta_i\otimes v_i$. 
\end{proof}

%{\bf Remark} Note that the lifts of relative cycles defined above are not well-defined at the level of corresponding relative homology class: the lifted cycles are only equivalent up to homology and cycles on the boundary component at infinity. In particular, if the map $H_1(\pl\ovl M;V_\ZZ)\to H_1(M;V_\ZZ)$ were surjective on the free part (which is not the case in general) we would generate the free homology by lifting relative cycles mapping to the trivial class.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Eisenstein integrals on boundary cells}

\begin{lemma}
There is a $N$ as in the statement of the proposition such that if $\omega$ is an holomorphic form representing an integral class in $H^1(\pl\ovl M; V_\CC)$ then we have 
$$
\langle E^1(\omega),i_*c \rangle \in N^{-1}\ovl\ZZ
$$
for all $c\in H_1(\pl\ovl M;V_{\ovl\ZZ})$.
\label{intbd}
\end{lemma}

\begin{proof}
The homotopy classes of loops on the component $T_j=\Lambda_j\bs N_j$ of $\pl\ovl M$ are represented by closed 1-parameter subgroups of $T_j$, which correspond to rational points $\LN_{j,\QQ}$ of the Lie algebra of $N_j$. Suppose for the moment that $f\in\Omega^1(M)$. Let $X\in \LN_{j,\ZZ}$ be a primitive vector (i.e. not multiple of another integer vector) and $X_0\in \LN_0,\, \gamma\in\SL_2(F)$ such that $X=\ad(\gamma)X_0$; let $g_\infty\in\SL_2(\CC)$ and let $c$ be the simple cycle which is the image of 
$$
\tilde c = \{\exp(tX)g, t\in\RR\}
$$
in $M$. Let $\tilde f$ be the function in $(C^\infty(\SL_2(\Ade))\otimes\LP^*)^{K'}$ corresponding to $f$ (see \eqref{eis}), and $\phi_0=\tilde f(\cdot)(X_0)\in C^\infty(\SL_2(\Ade))^{K_f'}$, then we have that 
$$
\int_c f = \int_0^1 f(\exp(tX)g_\infty)(X) dt = f(g_\infty)(X) = \phi_0(g_\infty g_f). 
$$
where $\SL_2(\Ade_f)\ni g_f\in\gamma K_f'$. Now if $f\in\Omega^1(M;V_\CC)$ and $v\in V_\CC$ we can apply the above argument to the $1$-form $\langle \rho\cdot f,v\rangle_V$ and it follows that 
$$
\int_c \langle \rho\cdot f,v\rangle_V = \phi_0(g_\infty g_f)
$$
as above. 

If $f$ is an Eisenstein series then $\phi_0$ above belongs to the subspace $C^\infty(\N(\Ade)\B(F)\bs\SL_2(\Ade))$, and in fact equals $\phi_s + (\Psi(s)\phi)_{-s}$ for some $\phi\in\sh$. For a closed form $E^1(\omega)$, $\omega\in H^1(\pl\ovl M;V_\CC)$ we get $\phi_0=\phi+\Psi(s_V^1)\phi$ (the integral against a cycle does not depend on the height in the cusp). Now if $\omega$ is integral, the function $\phi$ takes integral values when $v\in V_{\ovl \ZZ}$; thus we have translated our original problem of estimating the denominator of $E^1(\omega)$ for $\omega$ an harmonic $1$-form on $\pl\ovl M$ whose integrals against integral $1$-cycles is integral into the problem of estimating the denominator of the values of $\Psi(s_V^1)\phi$ for $\phi\in\sh^{K_f'}$ taking integral values on $K$. 

We thus want to prove that whenever $\phi\in\sh^{K_f'}$ takes integral values there is a $N$ with absolute norm $N_0\le C|\fri|^c$ such that $N\Psi(s_V^1)\phi$ takes integral values. We will prove this only for $\phi\in\sh(\chi)^{K_f'}$ where $\chi$ is a Hecke character with conductor dividing $\fri$; the general result follows since these $\phi$ generate $\sh^{K_f'}$; moreover we will suppose that $K_f'=K_f(\fri)$ (which is also not a problem in view of Lemma \ref{index-level}). Let $S_\fri$ be $\infty$ together with all finite places such that $K_f'$ is not maximal at $v$, i.e. $\fri\so_v=\pi_v^{m_v}\so_v$ for a $m_v\ge 1$. Then we have seen that 
\begin{equation}
\Psi(s)\phi = \prod_{v\in S_\fri} I_v \times \frac{L(\chi,2s-1)}{L(\chi,2s)}
\label{icicomp}
\end{equation} 
The values of $\chi_v$ on $\so_v^\times,\pi_v$ are algebraic numbers whose denominators and numerators have absolute norms bounded by $Cq_v^b$ where $b,C$ depend only on $\chi_\infty$ and $F$, and it follows easily from the computations of the local integrals given in \ref{ramify} (which until the last steps are valid for any $\phi_v$ and not only the specific choice made there; see also \cite[p. 145]{thesis}) that we have 
$$
I_v = \frac{L_v(\chi,s_V^1)}{L_v(\chi,s_V^1-1)} \Psi_v(s_V^1)\phi_v(k) \in C^{-1}q_v^{-cm_v}\ovl\ZZ
$$
for all $k\in K_v$ and some rational integers $C,c$ depending only on $F,V$ (where the quotient of local $L$-factors equals one when $\chi$ ramifies at $v$). It follows from\eqref{icicomp} that 
$$
\Psi(s)\phi(k) \in \Psi_\infty(\phi_\infty)(k_\infty)\frac{L(\chi,s_V^1-1)}{L(\chi,s_V^1)} C^{-1} |\fri|^{-c} \ovl\ZZ.
$$
The key ingredient now is the result of Damerell \cite{Damerell} about special values of Hecke $L$-functions, a corollary of which (as we explain in \ref{dame} below) is that there exists rational integers $m,M\in\ZZ$ and some number $\Omega\in\CC^\times$ depending on $F,V$ such that the $L$-values $L(\chi,s_V^1-1),L(\chi,s_V^1)$ belong to $\Omega\pi\ovl\QQ, \Omega\ovl\QQ$ respectively and the denominators of $L(\chi,s_V^1-1)/(\Omega\pi),L(\chi,s_V^1)/\Omega$ both divide $M|\frf_\chi|^m$. This yields 
$$
\Psi(s)\phi(k) \in \Psi_\infty(\phi_\infty)(k_\infty) \left(\pi C|\fri|^c\right)^{-1} \ovl\ZZ.
$$
Now we know that $\Psi(s)$ is defined over $\ovl\QQ$ and it follows that $\Psi_\infty(\phi_\infty)(k_\infty)\in\pi\ovl\QQ$, and as the component at infinity lives in a finite-dimensional space that does not depend on $\fri$ this finishes the proof\footnote{One can likely compute the term at the infinite place more precisely to see directly that it belongs to $\pi m^{-1}\ovl\ZZ$ for some $m\ge 1$ depending only on $V$.}.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Reduction to modular symbols}

There are two issues while computing the denominators of Eisenstein integrals against lifted cycles: some which come from the Eisenstein cohomology class itself and some that come from the cycle. One can quantify the latter by using so-called denominators of modular symbols (as is done in \cite{CV}) and then eschew them by expressing a given modular symbol as a sum of others to kill primes dividing the denominators (this is precisely expressed in \cite[6.7.4, ($\heartsuit$)]{CV}). Here we will use a more direct approach by using the following fact. 

\begin{lemma}
There is a $c>0$ depending only on $\Gamma$ such that any congruence subgroup of $\Gamma$ of level $\fri$ is generated by matrices whose coefficients are all smaller than $|\fri|^c$. 
\label{bd_gen}
\end{lemma}

\begin{proof}
To prove this, let $X$ be the Cayley graph of $\Gamma=\SL_2(\so_F)$ for some fixed generating system and $|\cdot|$ the word length on $\Gamma$ for the same. Then there exists a $C>0$ such that for every ideal $\frj$ of $\so_F$ there exists a finite subset $D_\frj\subset X$ such that $\Gamma(\frj)\cdot D_\frj = X$ and the diameter of $D_\frj$ is $\le C\log|\frj|$; this is equivalent to the fact that the diameter of the Schreier graphs of $\Gamma/\Gamma(\frj)$ with respect to a system of generators of $\Gamma$ are of diameter $\asymp\log|\frj|$ (which itself follows from the solution to conjecture $\tau$ which implies that they are an expanding family). We will denote by $v_0$ the vertex corresponding to the identity in $X$, so that $|\gamma|=d_X(v_0,\gamma v_0)$ for all $\gamma\in\Gamma$. Since the congruence subgroup $\Gamma'$ of level $\fri$ is generated by the set of those $\gamma\in\Gamma'$ such that $d(\gamma v_0, D_\fri)\le 1$ we see that we have:
\begin{equation}
\Gamma' = \langle \gamma\in\Gamma':\: |\gamma|\le C\log|\fri|\rangle.
\label{genbd}
\end{equation}
Now $X$ is quasi-isometric to the universal cover $Z$ of the truncated manifold $M^1$ via the map $\gamma v_0\mapsto \gamma x_0$ where $x_0$ is the fixed point of $\SU(2)$ in $Z\subset\HH^3$. Since the distance between two points in $Z$ is larger than the corresponding distance in $\HH^3$ we get that there is a $\delta>0$ such that 
$$
|\gamma| = d_X(v_0,\gamma v_0) \ge \delta d_{\HH^3}(x_0,\gamma x_0).
$$
Since the right-hand side is itself $\asymp\log\|\gamma\|$ where $\|\cdot\|$ is the Euclidean norm on $\SL_2(\CC)$ (such that elements of $\SU(2)$ have norm 1), our claim follows from \eqref{genbd}.
\end{proof}


\begin{lemma}
There are a $C,c$ depending on $F$ such that up to a integral factor with absolute norm less than $C|\fri|^c$, the denominator of an Eisenstein cohomology class $\phi\in H^1(M;V_{\ovl\QQ})$ is equal to the lowest common multiple of the denominators of all integrals $\langle \phi,c_{\xi,\gamma}\otimes v\rangle$ for any $\xi\in\PP^1(F)$, where $\gamma,v$ range in a generating set for $\Gamma$ and in $V_{\ovl\ZZ}$ respectively.
\label{killarc}
\end{lemma}

\begin{proof}
Let $\gamma_1,\ldots,\gamma_r$ be a generating set for $\Gamma'$ and $c_1,\ldots,c_r$ the corresponding loops in $M$ (based at some point $x_0$). It follows from the computation of $H_*(M;V_{\ovl\ZZ})=H_*(\Gamma;V_{\ovl\ZZ})$ by the bar-resolution that the homology is generated by those cycles which are of the form $\sum_{i=1}^rc_i\otimes v_i$ for $i=1,\ldots,r$ and $(v_i)\in V_\ZZ^r$. By Lemma \ref{mod_gen} for any $\xi\in\PP^1(F)$ these cycles are homologous, up to integral boundary closed 1-cells, to sums of the form
$$
\sum_{i=1}^r c_{\xi,\gamma_i}\otimes v_i + s_i\otimes v_i
$$
where $s_i$ is the geodesic segment on the boundary between the endpoints of $C_{\xi,\gamma_i}$. We can view $s_i$ as an element of the vector space $\Lambda\otimes_\ZZ\QQ$ where $\Lambda=\stab_{\Gamma'}\xi$; there is a $M\in\NN$ such that $Ms_i$ is closed and the lemma will follow (by applying Lemma \ref{intbd}) if we can estimate $M\le C|\fri|^c$ for $i=1,\ldots,r$. 

We will do this only for $\xi=\infty$; the general case is similar and not needed for the sequel (since we can work with any given $\xi$ alone). A direct computation shows that if 
$$
\gamma_i = \begin{pmatrix} a_i&b_i\\c_i&d_i\end{pmatrix}
$$ 
then $b_is_i$ is closed: indeed, it suffices to evaluate the denominator of $\gamma_i\infty-\gamma_i^{-1}\infty\in F$, which is equal to $(a_i+d_i)/b_i$. Since by Lemma \ref{bd_gen} we can generate $\Gamma'$ by elements with coefficients $\ll|\fri|^c$, the result follows.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Eisenstein integrals over $c_{\xi,\gamma}$}

In view of Lemmas \ref{mod_gen}, \ref{killarc} and \ref{intbd}, Proposition \ref{inteis} follows from the next statement.

\begin{lemma}
There is an $N$ as in the statement of Proposition \ref{inteis} such that for all $\omega\in H^{1,0}(\pl\ovl M;V_{\ovl\ZZ})$, $\xi\in\PP^1(F),\gamma\in\Gamma'$ and $v\in V_{\ovl\ZZ}$ we have
$$
\langle E^1(\omega), c_{\xi,\gamma}\otimes v\rangle \in N^{-1}\ovl\ZZ.
$$
\label{intmod}
\end{lemma}

\begin{proof}
We follow Calegari and Venkatesh \cite[6.7.6]{CV}. We fix a nontrivial additive character $\psi$ of $\Ade/F$ so that the Haar measure is self-dual for $\psi$. Let $v\in V_{\ovl\ZZ}$; there is a $f\in\sh$ such that the $1$-form $\langle E^1(\omega),v\rangle$ corresponds to $E(f_{s_V^1})$ under the identification of \eqref{eis}. We may suppose that $f\in\sh(\chi)$ for some Hecke character whose infinite part belongs to a finite set (determined by $V$) and which has a conductor dividing $\fri$. For $\gamma\in\Gamma$ and $\xi\in\PP^1(F)$ we have:
\begin{equation}
\int_{c_{\xi,\gamma}} \langle E^1(\omega),v\rangle = \frac 1{h_F} \sum_{\omega} \int_{\T(F)\bs\T(\Ade)} \omega(t)E(f_{s_V^1})(tg_f) dt
\label{int_no1}
\end{equation}
where: 
\begin{itemize}
\item $g_f$ is an element in $\G(F)$ which sends $(0,\infty)$ to $(\xi,\gamma\xi)$; 
\item the sum is over all characters $\omega$ of the class-group of $\T$ (which is isomorphic to the class-group of $F$);
\item The Haar measure $dt$ on $\T(\Ade)$ has a certain normalization which depends only on $F$ (see \cite[5.3.3]{CV}).
\end{itemize}
The so-called Whittaker function at $v$ of $f$ is defined by:
$$
W_v(g) = \int_{\N(F_v)} f_v(wng)\psi(n) dn
$$
and $W$ by $\prod_v W_v$; we then have the Fourier expansion
$$
f(g) = f_P(g) + \sum_{a\in\T(F)} W_v(ag). 
$$
Since the part of \eqref{int_no1} corresponding to the constant term vanishes, it follows that
$$
\int_{c_{\xi,\gamma}} \langle E^1(\omega),v\rangle = \frac 1{h_F}\sum_{\omega} \int_{\T(\Ade)} W(tg_f) \omega(t) dt 
$$
Now let $S$ be the set of finite places such that either:
\begin{itemize}
\item $K_f'$ is not maximal at $v$;
\item or $g_v\not\in K_v$. 
\end{itemize}
Then for $v\not\in S$ we have 
\begin{equation}
\int_{\T(F_v)} W(t_vg_v)\omega(t_v) dt_v \in \frac {L_v(\chi\cdot\omega,s_V^1+1/2)\cdot L_v(\ovl\chi\cdot\omega,s_V^1+1/2)}{D_v L_v(\chi^2,1+2s_V^1)} \ovl\ZZ
\label{unramified}
\end{equation}
(see \cite[6.7.6.3]{CV}, which we apply to the non-unitary character $|\cdot|_v^{s_V^1}\chi$). In general we have 
\begin{equation}
\int_{\T(F_v)} W(t_vg_v)\omega(t_v) dt_v \in q_v^{-m} \frac {L_v(\chi\cdot\omega,s_V^1+1/2)\cdot L_v(\ovl\chi\cdot\omega,s_V^1+1/2)}{D_v L_v(\chi^2,1+2s_V^1)} \ovl\ZZ
\label{ramified}
\end{equation}
for some integer $m$ (see \cite[Proposition 4.7.5]{Bump}), and since the function $t_v\mapsto W_v(t_vg_v)$ is $1+\pi_v^{k+l}\so_v$-invariant (where $K_v'$ is of level $\frp_v^k$ and $l$ is the distance in the Bruhat--Tits tree between $\T(F_v)g_v$ and the fixed point of $K_v$) it is clear from the nature of the computations that $m\ll k+l$. So putting together \eqref{ramified} and \eqref{unramified} we finally get that for some $c\in\NN$ we have:
$$
\int_{c_{\xi,\gamma}} \langle E^1(\omega),v\rangle \in |\fri|^{-c} |\frj|^{-c} \frac{L(\chi\cdot\omega,s_V^1+1/2)\cdot L(\ovl\chi\cdot\omega,s_V^1+1/2)}{h_FD_F L(\chi^2,1+2s_V^1)} \ovl\ZZ
$$
where $\frj$ is the larger ideal such that $\gamma\in\Gamma(\frj)$. It follows from Damerell's theorem that we have 
$$
\frac{L(\ovl\chi\cdot\omega,s_V^1+1/2)}{L(\chi^2,1+2s_V^1)} \in |\fri|^{-c'}\ovl\ZZ
$$
for some $c'$ (depending only on $s_V^1$), hence
$$
\int_{c_{\xi,\gamma}} \langle E^1(\omega),v\rangle \in \frac 1{h_FD_F} |\fri|^{-c'-c} |\frj|^{-c} \ovl\ZZ. 
$$
To finish the proof of the lemma it suffices to remark that we can restrict to a generating set for the range of $\gamma$ we need to consider, and to apply Lemma \ref{bd_gen}. 
\end{proof}

%{\bf Remark} To prove Lemmas \ref{killarc} and \ref{intmod} we could have used the approach of \cite{CV} using the `denominators' of modular symbols rather than a family of generators. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Damerell's theorem}
\label{dame}
To state this result precisely we need some notation. Let $E$ be the Hilbert class field of $F$: it is a finite abelian extension of $F$ such that for every ideal $\fri$ of $F$, $\fri\so_E$ is a principal ideal of $\so_E$. We will denote $m_\fri$ a generator for this ideal (an ``ideal number'' of $\fri$ in Damerell's paper). Damerell's result \cite[Theorem 2]{Damerell} implies that there exists some $\Omega\in\CC^\times$ which depends only on $F$ such that if $s\in\frac 1 2\ZZ$ and we put
$$
\gamma = 6 m_\fri^{2s}|\fri|^{\frac s 2}
$$
for an ideal $\fri$ then for any Hecke character $\chi$ such that $\frf_\chi$ divides $\fri$ we have that 
\begin{equation}
\gamma \frac{L(\chi,s)}{\Omega^{2s}}\in\ovl\ZZ \text{ and } 2\gamma\pi \frac{L(\chi,s-1)}{\Omega^{2s}} \in\ovl\ZZ.
\label{dalek}
\end{equation}
The absolute norm of the ideal $\fri\so_E$ equals $|\fri|^{[E:F]}$ and we thus see that \eqref{dalek} implies the result stated in the proof of Proposition \ref{inteis} above.



